Scalable adaptive PDE solvers in arbitrary domains

Efficiently and accurately simulating partial differential equations (PDEs) in and around arbitrarily defined geometries, especially with high levels of adaptivity, has significant implications for different application domains. A key bottleneck in the above process is the fast construction of a `good' adaptively-refined mesh. In this work, we present an efficient novel octree-based adaptive discretization approach capable of carving out arbitrarily shaped void regions from the parent domain: an essential requirement for fluid simulations around complex objects. Carving out objects produces an $\textit{incomplete}$ octree. We develop efficient top-down and bottom-up traversal methods to perform finite element computations on $\textit{incomplete}$ octrees. We validate the framework by (a) showing appropriate convergence analysis and (b) computing the drag coefficient for flow past a sphere for a wide range of Reynolds numbers ($\mathcal{O}(1-10^6)$) encompassing the drag crisis regime. Finally, we deploy the framework on a realistic geometry on a current project to evaluate COVID-19 transmission risk in classrooms.

==> Applications.tex <==
This work is motivated by applications that requires adaptive octrees for discretizing long channels or complex geometries. In such cases, the traditional method of generating octree fails on account of their symmetric nature in all the dimension. Our target applications involve simulating the Navier--Stokes equations in three scenarios of increasing complexity: a) flow across a single complex object for a very wide range Reynolds numbers ($Re$); b) flow across a stack of identical objects representing a packed-bed biomedical microfluidic device; and c) flow across a stack of complex heterogeneous objects representing virus transmission in an occupied classroom. These canonical applications exemplify the difficulty of anisotropic geometries as well as presence of multiple complex objects in the simulation domain. %All these applications either have a long channel or complex objects or combination of both.

\subsubsection{LES simulation over complex objects}
Traditionally, unstructured body conforming grid was used to solve the Navier--Stokes equation over complex geometries. The generation of these analysis-suitable,  body-fitted mesh with appropriate refinement near the geometry is usually a time consuming and labor intensive process. Immersed boundary method (IBM) tends to alleviate these time consuming laborious process and no longer requires the body conforming meshes. In the past, we have successfully deployed Immersogeometric analysis (IMGA, IBM variant within FEM context), on a massively parallel octrees and shown the ability to capture the flow physics accurately \cite{saurabh2020industrial}. 

Although these methods have been shown to accurately capture the flow physics across a wide range of $Re$, they come at an additional cost of performing a surface loop over the geometry, to account for the immersed geometry ~\citep{saurabh2020industrial,xu2016tetrahedral,xu2019immersogeometric}. In order to successfully deploy IMGA, the surface discretization of the geometry must ensure that each background \Intercepted elements must contain at least 3-4 surface quadrature points. This overhead increases substantially with increase in the level of refinement of the background mesh and becomes a bottleneck especially for high $Re$ flow which inherently requires a very refine region close to the body in order to accurately capture the flow physics.  We refer the interested reader to ~\citet{saurabh2020industrial} for a detailed discussion on deployment of IMGA on octrees. We note that, with an increase in the refinement near the object, the voxelated \textit{carved} out geometry asymptotically approaches the actual geometry. As shown in \figref{fig: ProjectedArea} for a sphere, the projected area \footnote{Projected area is chosen as a measure at it plays an important role in determining the aerodynamic coefficient.} of the voxelated sphere asymptotically converges to the theoretical value. Thus, for applications where the inherent physics requires a fine resolution near the boundaries, e.g. the cases with thin boundary layers, using a \textit{carved} geometry becomes a viable choice to accurately perform the flow simulation.
\input{Plots/ProjectedArea}
\input{Plots/signedDistance}

\subsubsection{Lab on a chip devices}
With recent advances in fabrication process and 3D printing, high throughput microfluidic devices, capable of performing multiplexed laboratory analysis at a miniaturized scale have gained increasing interest \cite{waheed20163d}. These devices offer a multitude of advantages, like high throughput and efficiency, low production cost, low power consumption, parallel processing of samples, and fast sampling times. They are characterized by device geometries that exhibit extremely skewed aspect ratios (for instance, $1\times64\times 1024$), and with multiple objects within the device \cite{boy2008simulation}. This make octrees an attractive choice to simulate such devices. However, the skewed channel dimensions make it hard to deploy traditional octree approaches. Further, the presence of objects, such as sphere or pillar (to enhance the pressure drop, thus increasing the throughput ~\cite{zhao2017high} or get the desired focusing pattern ~\cite{kommajosula2019high,liu2017high,stoecklein2016optimization}) makes it even harder to mesh and simulate these devices.

\subsubsection{Simulation of Covid transmisson in classroom}
The COVID-19 pandemic has wreaked havoc on educational institutions. Best practice guidelines for safe in-person teaching is critical to ensure safe learning. In this context, high fidelity fluid simulations are a practical approach to evaluate various seating and operating scenarios~\citep{covid2020operating,wu2020effects}, identify risk factors, and rank order mitigation strategies. The availability of a fast mesh generation tool that can efficiently account for complex objects can significantly enable decision making by providing workflows that are rapidly deployable, personalized to specific room/scenario, and easy to extract reliable best practices.

%Most current simulation strategies utilize simplified assumptions for modeling the flow and aerosol distribution. We have exciting preliminary work that integrates four sophisticated concepts to provide very detailed estimates of aerosol distribution in indoor environments: (a) a detailed flow physics simulation (called Large Eddy Simulations) that produces significantly more accurate results while taking reasonable compute time, (b) accounting for the thermal plumes created by heat released by humans and electronics (which changes the flow in rooms), (c) immersogeometric analysis (see figures attached) that allows rapid exploration of a diverse array of configurations with complex geometries, (d) a detailed microdroplet distribution model that accounts for the distribution of droplet size due to evaporation, coalescence and breakup. There has not been any such high fidelity simulations performed to our best knowledge. 

%After the Covid pandemic hit United States in the March of 2020, the schools and colleges shut down. Many of the colleges did open in Fall for in-person classes, but some of them had to later shut down due to spike in the number of Covid cases. It remains an open question to how to safely open the colleges for in--person classes. The transmission of coronavirus in a classroom can be affected by a variety of factors like the sitting arrangements between the students in the classroom, the ventilation of the classroom or the humidity level ~\citep{covid2020operating,wu2020effects}. T

==> DragCrisis.tex <==
\subsection{Validation case: Simulating drag crisis for flow past a sphere}\label{sec: DragCrisis}

% \input{Plots/SphereDrag}
\input{Plots/DragCombined}
We validate our numerical setup for Navier--Stokes simulation by computing the non-dimensional drag coefficient $C_d$ on sphere across a range of Reynolds number from 1 to 2,000,000. A sphere of diameter $d=1$ is placed at a distance $3d$ from the inlet at $(3d, \,3d,\, 3d)$ in a computation domain of $(10d, \,6d,\, 6d)$. The walls of the domain, except the outlet have constant non-dimensional freestream velocity of $(1, \, 0, \, 0)$ and zero pressure gradient. At the outlet, the pressure is set to 0 and zero gradient velocity boundary condition is applied at the wall. The no-slip boundary condition (zero Dirichlet) for velocity is imposed on the surface of sphere. The mesh resolution for the octree is varied depending on the Reynolds number and according to the Taylor's micro length scale. 
% In order to capture the curvature of the sphere accurately, the refinement level near the sphere was not dropped below 12 (\figref{fig: ProjectedArea}). 
Equivalently depending on the Reynolds number, the mesh in the wake region was refined to capture the turbulent structures. The spatial domain was discretized using linear basis function and the Crank Nicholson scheme was used for temporal discretization. 



\figref{fig: Drag} shows the variation of $C_d$ across the range of Reynolds number. We see that the results are in excellent agreement with the experimental result. It must be noted that we are able to accurately capture the drag crisis phenomena, where a sudden drop in drag from 0.5~\citep{achenbach1972experiments} - 0.6~\citep{bakic2003experimental} at Re around $16,000$ to 0.1~\citep{achenbach1972experiments} - 0.2~\citep{geier2017parametrization} at $Re$ of 2 million is observed. \added{~\figref{fig: SphereDragHighRe} shows the variation of $C_d$ with $Re$ on semi-log axis close to the drag crisis regime and compares with other numerical and experimental results from literature. We can see that our numerical results are in good agreement. Our finest resolution consists of around 40M elements which is close to the medium resolution for LBM simulation as done by ~\citet{geier2017parametrization}. No finer resolution is needed (or considered due to the high computational cost).} 

The prediction of drag crisis is of significant interest to the CFD community, with important engineering implications in aerodynamics and vehicular dynamics. We emphasize that no special numerical/modelling treatment is needed in this framework to capture the drag crisis; this is in contrast to existing work where typically a wall treatment~\citep{hoffman2006simulation,constantinescu2004numerical} is required to predict the drag crisis.


\figref{fig: wake} shows the turbulent flow structures with increasing $Re$. At $Re = 10,000$, the boundary layer becomes turbulent \figref{fig: Re10K}. With increase in $Re$, the vortices becomes smaller but the separation angle is not affected ($Re=160,000$ \figref{fig: Re160K}) until the critical regime is reached. \figref{fig: wake} gives the phenomenological description of drag crisis, which is evident by noticing the wake structure between \figref{fig: Re160K} at $Re=160K$ (subcritical regime) and \figref{fig: Re2M} at $Re=2\times 10^6$ (supercritical regime). In the subcritical regime, the wake behind the sphere tends to diverge as it moves away from the sphere. Above the critical $Re$, the wake tends to converge and become narrower as it moves behind the sphere. Subsequently, we can observe a high pressure zone being developed behind the sphere. The main reason for the drag crisis can be attributed to the development of this high pressure zone behind the sphere that tends to push the sphere in the inflow direction. These results are in agreement with the simulations by~\citet{geier2017parametrization} using Lattice Boltzmann method to capture the drag crisis.

\input{Plots/sphereDragLinear}


==> Plots/COVIDClassroom.tex <==
% \begin{figure*}[t!]
% \centering
% \begin{subfigure}{.5\textwidth}
%     \includegraphics[width=1.0\linewidth]{Images/COVID-Classroom-1.png}
%     \caption{Computational domain, boundary condition and enlarged mesh slice}
%     \label{fig: COVIDClassroom_1}
% \end{subfigure}
% \\
% \begin{subfigure}{.44\textwidth}
%     \includegraphics[width=1.0\linewidth]{Images/COVID-Classroom-2.png}
%     \caption{Flow structure and streamlines}
%     \label{fig: COVIDClassroom_2}
% \end{subfigure}
% \vspace{1mm}
% \caption{\textit{Classroom simulation}: ~\figref{fig: COVIDClassroom_1} shows the computation domain of complex geometries in a rectangular domain. The computation domain consists of a cuboid domain of $4.86 \times 3.34 \times 1 $, with 6 sets of tables, chairs and sitting mannequins as well as 1 standing mannequin represented by STL files. ~\figref{fig: COVIDClassroom_2} shows one vertical slice of line integral convolution plot around the middle plane of the classroom and streamlines from the around the head region of one student.}
% \label{fig: COVIDClassroom}
% \end{figure*}

% \begin{figure}
% % \vspace{-5mm}
%     \includegraphics[width=0.00\linewidth]{Images/COVID-Classroom-1.png}
%     \caption{Figure showing the computational domain, boundary condition and enlarged mesh slice for the classroom simulation. The computation domain consists of a cuboid domain of $4.86 \times 3.34 \times 1 $, with six sets of tables, chairs and sitting mannequins as well as one standing mannequin represented by STL files.}
%     \label{fig: COVIDClassroom_1}
% \end{figure}

% % \vspace{-5mm}
% \begin{figure}
%     \includegraphics[width=0.99\linewidth, trim=30 0 80 0, clip]{Images/COVID-Classroom-2.png}
%     \caption{Figure showing one vertical slice of line integral convolution plot around the middle plane of the classroom and streamlines from around the head region of one student}
%     \label{fig: COVIDClassroom_2}
% \end{figure}

==> Plots/MicrofluidPackedBed.tex <==
% \begin{figure*}
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1.0\linewidth, trim=0 0 200 0]{Images/packedBedSlice.png}
%   \caption{Velocity streamlines over multiple spheres packed in micro channel}
%   \label{fig:micro-channelVelocity}
% \end{subfigure}
% \newline
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include second image
%  \begin{tikzpicture}
% \begin{axis}[
%           %width=0.6\linewidth, % Scale the plot to \linewidth
%           width=0.5\linewidth,
%           %height=0.2\textwidth,
%           %grid=major, % Display a grid
%           %grid style={line width=.1pt, draw=gray!50}, % Set the style
%           xlabel=Z, % Set the labels
%           ylabel= Pressure,
%           ymin = 0.0,
%         %   ymax = 12.0,
%           xmin=0,
%           legend style={at={(1.2,0.7)},anchor=north west,legend columns=1}, % Put the legend below the plot
%           x tick label style={rotate=0,anchor=north}, % Display labels sideways
%           legend style={at={(0.55,0.95)},anchor=north west,legend columns=1}, % P % Put the legend below the plot
% 			]
% 	  \addplot [no marks, dashed] gnuplot [raw gnuplot, color=red,ultra thick] {
%       set datafile separator ",";
%       plot "Data/PressurePlotNoSphere.csv" using ($1):($2) with lines
%      };
% 	  \addplot [no marks] gnuplot [raw gnuplot, color=black,ultra thick] {
%       set datafile separator ",";
%       plot "Data/PressurePlot.csv" using ($1):($2) with lines
%      };
      
%       \legend{\small Without spheres,\small With spheres}
			
% \end{axis}
% \end{tikzpicture}
%   \caption{Pressure drop across the center line of channel in presence of spheres in a microchannel.}
%   \label{fig:pressureDrop}
% \end{subfigure}
% \caption{Velocity profile and pressure drop in case of packed bed micro channel}
% \label{fig:wake}
% \end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth, trim=0 0 200 0]{Images/packedBedSlice.png}
%     \caption{Velocity streamlines over multiple spheres packed in micro channel}
%     \label{fig:vmagPackedBed}
% \end{figure}

\begin{figure*}[t!]
\centering
\begin{subfigure}{.32\textwidth}
    \includegraphics[width=0.99\linewidth]{Images/packedBedSetup.png}
    \caption{Microfluidics setup}
    \label{fig:packedBed}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \includegraphics[width=0.99\linewidth,trim=0 0 200 0]{Images/packedBedSlice.png}
   \caption{Velocity streamlines of flow over multiple spheres packed in micro channel}
   \label{fig:micro-channelVelocity}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
\hspace{5 mm}
\begin{tikzpicture}
\begin{axis}[
          %width=0.6\linewidth, % Scale the plot to \linewidth
          width=0.9\linewidth,
          %height=0.2\textwidth,
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=Channel length (Z), % Set the labels
          ylabel= Pressure ($\times 10^3$),
          ymin = 0.0,
          xmin=0,
          legend style={at={(1.1,0.8)},anchor=north west,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north}, % Display labels sideways
          legend style={at={(0.45,0.95)},anchor=north west,legend columns=1}, % P % Put the legend below the plot
			]
	  \addplot [no marks, dashed] gnuplot [raw gnuplot, color=red,ultra thick] {
      set datafile separator ",";
      plot "Data/PressurePlotNoSphere.csv" using ($1):($2/1000) with lines
     };
	  \addplot [no marks] gnuplot [raw gnuplot, color=black,ultra thick] {
      set datafile separator ",";
      plot "Data/PressurePlot.csv" using ($1):($2/1000) with lines
     };
      
      \legend{\footnotesize{Without spheres},\footnotesize{With spheres}}
			
\end{axis}
\end{tikzpicture}
\caption{Pressure drop along the channel length}
\label{fig:pressureDrop}
\end{subfigure}

\vspace{1mm}
\caption{\textit{Microfluidics simulation}: \figref{fig:packedBed} shows the computation domain of spheres packed in a microchannel. The computation domain consists of a cuboid domain of $16 \times 1 \times 128 $, with 10 layers of 26 spheres each (diameter = 0.8) packed in a Body Centered Cubic (BCC) pattern. \figref{fig:micro-channelVelocity} shows the velocity streamlines over multiple spheres packed in micro channel. \figref{fig:pressureDrop} compares the enhanced pressure drop in presence of spheres along the channel length. }
\label{fig: microfluid}
\end{figure*}

==> Plots/packedBedSetup.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Images/packedBedSetup.png}
%     \caption{\textit{Packed bed-microfluidics:} Figure showing the computation domain of spheres packed in a microchannel. The computation domain consists of a cuboid domain of $16 \times 1 \times 128 $, with 10 layers of 26 spheres each (diameter = 0.8) packed in a Body Centered Cubic (BCC) pattern.}
%     \label{fig:packedBed}
% \end{figure}

==> classroomAE.tex <==
\subsection{Classroom Simulation: Computational Domain and Boundary Conditions}
\label{sec:classroomAE}

\figref{fig:classroomDomain} shows the computational domain that includes complex features such as tables, chairs and mannequins representing students and instructor. The velocity inlets and pressure outlets are located at the top of the domain. 
\subsubsection{Navier--Stokes simulation:\;}
The computational domain is $4.83 \times 3.34 \times 1$, the non-dimensional inlet velocity is $(0, 0, -1)$ at velocity inlets and zero pressure outlet on the side of the domain. the remaining boundaries are no-slip velocity boundary. $Re = 10^5$ based on the inlet velocity and classroom height. This flow rates and room geometry represent typical values in classrooms seen in US schools and universities. 

\subsubsection{Advection--Diffusion equation:\;} Once an statitstically stationary state has been achieved, we use the averaged velocity field to solve the advection--diffusion equation (scalar transport).  The initial cough releases viral particles in a conical region near the mouth of the mannequin and is evolved using the advection diffusion equations.

